Preserving Pre-trained Representation Space: On Effectiveness of Prefix-tuning for Large Multi-modal Models

Recently, we have observed that Large Multi-modal Models (LMMs) are revolutionizing the way machines interact with the world, unlocking new possibilities across various multi-modal applications. To adapt LMMs for downstream tasks, parameter-efficient fine-tuning (PEFT) which only trains additional prefix tokens or modules, has gained popularity. Nevertheless, there has been little analysis of how PEFT works in LMMs. In this paper, we delve into the strengths and weaknesses of each tuning strategy, shifting the focus from the efficiency typically associated with these approaches. We first discover that model parameter tuning methods such as LoRA and Adapters distort the feature representation space learned during pre-training and limit the full utilization of pre-trained knowledge. We also demonstrate that prefix-tuning excels at preserving the representation space, despite its lower performance on downstream tasks. These findings suggest a simple two-step PEFT strategy called Prefix-Tuned PEFT (PT-PEFT), which successively performs prefix-tuning and then PEFT (i.e., Adapter, LoRA), combines the benefits of both. Experimental results show that PT-PEFT not only improves performance in image captioning and visual question answering compared to vanilla PEFT methods but also helps preserve the representation space of the four pre-trained models.

==> equations/contrastive_loss.tex <==
\begin{equation}
\label{eqn:contrastive_loss}
L_{C} = - \displaystyle\sum_{(w,q,v)\sim D}\log{p(y|f(w,q,v))}.
\end{equation}

==> equations/image_caption_loss.tex <==
\begin{equation}
\label{eqn:image_caption_loss}
L_{IC} = - \displaystyle\sum_{(w,q,v)\sim D}\displaystyle\sum_{(i=0)}^{N}\log{p(w_i|w_{0},...,w_{i-1},q,v)}.
\end{equation}

==> equations/inter-domain_attention_score.tex <==
\begin{equation}
\label{eqn:inter-domain_atn_sc}
S_h[l,q,k] = \frac{1}{B} \frac{1}{N_q} \displaystyle\sum_{i\in q} \displaystyle\sum_{j\in k}  A_h [l,i,j]
\end{equation}

==> equations/masked_token_loss.tex <==
\begin{equation}
\label{eqn:MTL_loss}
L_{MTL} = - \displaystyle\sum_{(w,q,v)\sim D}\log{p(w_i|w_{i/},q,v)}.
\end{equation}

==> equations/rank_mul.tex <==
\begin{equation}
\label{eqn:representation_layer}
\text{rank}(Y) < \min({\text{rank}{(X)},\text{rank}{(W)}}).
\end{equation}

==> equations/representation_layer.tex <==
\begin{equation}
\label{eqn:representation_layer}
Y = XW + b.
\end{equation}

==> equations/svd_figure.tex <==
\begin{equation}
\label{eqn:image_caption_loss}
\displaystyle\sum_{(i=1)}^{N}\sigma_{i}.
\end{equation}

==> figures/P_adapter_BLIP.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{images/p-adapter1.pdf}
    \caption{\normalsize{BLIP-2 P-Adapter tuning SVD experiment.}}
    \label{fig:svd_ranks_blip_padater}
\end{figure}

==> figures/all_imts_correlation.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.55\textwidth]{images/imt_all_correlation.eps}
\caption{Cosine similarity map between all the IMTs of BVLT-n models in Table~\ref{tab:analysis_num}.}
\label{fig:imt_all_correlation}
\end{figure*}

==> figures/attention_maps.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{images/attention_maps/attention_map1.eps}
        \caption{}
        \label{fig:inter-atten-maps_a}
    \end{subfigure}\hfill
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{images/attention_maps/attention_map5.eps}
        \caption{}
        \label{fig:inter-atten-maps_b}
    \end{subfigure}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{images/attention_maps/attention_map9.eps}
        \caption{}
        \label{fig:inter-atten-maps_c}
    \end{subfigure}\hfill
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{images/attention_maps/attention_map12.eps}
        \caption{}
        \label{fig:inter-atten-maps_d}
    \end{subfigure}
    
    \caption{Average attention maps of the (a) 1st (b) 5th (c) 9th (d) 12th layers.}
    \label{fig:interdomain_attn_maps}
\end{figure}

==> figures/attention_mask.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{images/Attention_Mask_2.pdf}
\caption{Illustration of attention mask in WSA and ISA:  (a) attention mask of conventional VL model in  pre-training step, (b) attention mask of conventional VL model in fine-tuning step}
% , and (c) attention mask of IMT model in fine-tuning step.}
\label{fig:attention_mask}
\end{figure}


==> figures/concept_overeview.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{concept_overview.eps}
\caption{Comparison of inter-modality attention mechanism between conventional BERT based Vision-Language model and proposed [IMT] token based model. The blue arrow indicates the information flows through the self attention layers.
Note that inclusion of the tag is optional, since most of conventional models do not have tags in the input sequence.
Conventional model lost its image<-caption connection during the fine-tuning.
To address this problem, we introduce additional learnable latent vector [IMT] which map the image token sequence in a form to better attend with the caption sequence. }
\label{fig:concept_overeview}
\end{figure}

==> figures/dif_tag_num.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{dit_tags_num_attn.eps}
    \caption{M0 Model Metrics with the different numbers of image tags. The tags are sorted in descending order with confidence score, and included to experiment one by one.}
    \label{fig:dif_tag_num}
\end{figure}

==> figures/gen_inter_map.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{gen_inter_domain_attentionmap.eps}
    \caption{Conducted experiment for the analysis: object tag manipulation and inter-domain attention masking.}
    \label{fig:gen_inter_map}
\end{figure}

==> figures/imt_model.tex <==
\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\linewidth]{images/yesterday_fix.pdf}
\caption{Qualitative examples of image captioning and visual question answering tasks.}
%Note that for caption generation, only image tokens are considered (gray lines) on the left-side self-attention (LSA).}
\label{fig:imt_model}
\vspace{-0.3cm}
\end{figure*}

==> figures/imt_motivation.tex <==
% \begin{figure}[t!]
% \centering\includegraphics[width=\linewidth]{images/Motivation_2.eps}
% \caption{Illustration of the discrepancy between pre-training and fine-tuning steps of BERT-based VL model in image captioning: (a) pre-training step and (b) fine-tuning step of conventional BERT-based VL model.
% % (a) pre-training step of conventional BERT-based VL model and (b) fine-tuning step of conventional BERT-based VL model. 
% \textcolor{red}{Note that SA stands for self-attention. $\text{SA}_\theta$ is a single block used in two different ways where each takes word tokens $C$ and image tokens $I$ as query.}
% }
% \vspace{0.2cm}
% \label{fig:imt_motivation2}
% \end{figure}
\begin{figure*}[t!]
\centering\includegraphics[width=0.83\linewidth]{images/sharp_fix.pdf}
\vspace{-0.4cm}
\caption{Illustration of the representation space. $I$ and $C$ denote image feature vectors and word embedding vectors in the image captioning training. Prefix-tuning can preserve the learned representation space, and fine-tuning (i.e., full fine-tuning, LoRA) can further optimize the model for the task. CGFT takes advantage of both methods.}
\label{fig:imt_motivation}
\vspace{-0.4cm}
\end{figure*}


==> figures/imt_overview.tex <==
\begin{figure}[t!]
\centering\includegraphics[width=0.95\linewidth]{images/IMT_motivation_gap5.pdf}
\caption{Pre-training and fine-tuning strategies for VL tasks.}
\label{fig:imt_overivew}
\end{figure}


==> figures/interdomain_attn_maps.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{coco_captioning_base_xe_avg_attn.eps}
        \label{fig:inter-atten-maps_a}
    \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{nocaps_base_xe_avg_attn.eps}
        \label{fig:inter-atten-maps_b}
    \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{pretrained_avg_attn.eps}
        \label{fig:inter-atten-maps_c}
    \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{coco_captioning_base_xe_0_attn.eps}
        \label{fig:inter-atten-maps_d}
    \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{coco_captioning_base_xe_1_attn.eps}
        \label{fig:inter-atten-maps_e}
    \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{coco_captioning_base_xe_2_attn.eps}
        \label{fig:inter-atten-maps_f}
    \end{subfigure}
    
    \caption{Inter-domain attention map scores for different model configuration in table~\ref{tab:attn_map_model_metric}. (a), (b), (c) is inter domain attention map of M0, M1 and M2 Model respectively. Inter domain attention map is derived layer-by-layer in BERT with averaging multi head attention maps. (d), (e), (f) is inter domain attention map of the first, second and third layer of M0 model.}
    \label{fig:interdomain_attn_maps}
\end{figure}

==> figures/ofa_rank.tex <==
\begin{figure}[t!]
    % \caption{The ablation of PGF-tuning.}
    \setlength\heavyrulewidth{1.5pt}
    \renewcommand{\arraystretch}{1.0}
    \begin{subfigure}{0.48\textwidth}
    \centering
    % \resizebox{\linewidth}{!}{
    \includegraphics[width=0.8\linewidth]{images/ofa_svd_vqa_img.pdf}
    \caption{Image Representation}
    \end{subfigure} \vfill
    \begin{subfigure}{0.48\textwidth}
    \centering
    % \resizebox{\linewidth}{!}{
    \includegraphics[width=0.8\linewidth]{images/ofa_svd_vqa_txt.pdf}
    \caption{Text Representation}
    \end{subfigure}
    \caption{Acummulated and normalized singular values of feature vectors extracted from the last layer of OFA. The model is fine-tuned for COCO dataset.}
    \label{fig:svd_ofa}
    \vspace{-0.1cm}
\end{figure}

==> figures/tag_manipulation.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.94\linewidth]{images/Tag_manipulation2.eps}
\caption{Effect of the image tag manipulation on image captioning. For fully converged VINVL, the number of input tags varies with (a) actual image tags or (b) randomly selected tags.}
\label{fig:tag_manipulate}
\end{figure*}

==> figures/three_experiments.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.96\linewidth]{images/Tag_Ablation.pdf}
\caption{Three types of the experiments conducted for the tag-based VL model analyses. (a) The input structure of the tag based model. (b) Tag generating process with image features. (c) Tag ablations and inter-domain attention ablation settings.}
\label{fig:three_experiments}
\end{figure*}

==> figures/threeexperiments_foranalysis.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.25\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Randomtag.eps}
        \label{fig:inter-atten-maps_a}
    \end{subfigure}\hfill
    \begin{subfigure}{0.25\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Differentnumberoftag.eps}
        \label{fig:inter-atten-maps_b}
    \end{subfigure}\hfill
    \begin{subfigure}{0.35\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Interdomainmasking.eps}
        \label{fig:inter-atten-maps_c}
    \end{subfigure}\hfill
    \begin{subfigure}{0.3\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Interdomainmasking.eps}
        \label{fig:inter-atten-maps_d}
    \end{subfigure}\hfill
    \begin{subfigure}{0.3\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Interdomainmasking.eps}
        \label{fig:inter-atten-maps_e}
    \end{subfigure}\hfill
    \begin{subfigure}{0.3\linewidth}
        \caption{}
        \includegraphics[width=\linewidth]{images/Interdomainmasking.eps}
        \label{fig:inter-atten-maps_f}
    \end{subfigure}
    
    \caption{Performance Analysis on the components of Image tag-based VL model. (a), (b), (c) are the experiments on tag manipulation, and (d), (e), (f) are the three corresponding experiments using inter-domain masking.}
    \label{fig:interdomain_attn_maps}
\end{figure}

==> tables/BVLT_coco_with_others.tex <==
\begin{table}[t]
% \caption{Comparison with BASE size SoTA VL models on COCO image captioning dataset test split.} % \caption
\caption{Performance comparison of various BASE-sized VL models on COCO test split.}
\centering
\setlength\heavyrulewidth{1.5pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Model & Type & B4        & C          & S         \\ \midrule \midrule
Unified VLP~\citep{zhou2020unified} & BERT-based & 39.5 & 129.3 & 23.2 \\ \midrule
OSCAR~\citep{li2020oscar} & BERT-based & 40.5 & 137.6 & 22.8          \\ \midrule
VINVL~\citep{zhang2021vinvl} & BERT-based & 40.9 & 140.4 & \textbf{25.1} \\ \midrule
SimVLM~\citep{wang2021simvlm} & Enc-Dec & 39.0 & 134.8          & 24.0          \\ \midrule
X-VLM~\citep{zeng2021xvlm} & Enc-Dec & \textbf{41.3} & 140.8          & -             \\ \midrule\midrule
\textbf{P2F-1 (Ours)} & BERT-based & 41.1 & 141.0 & 25.0          \\ \midrule
\textbf{P2F-16 (Ours)} & BERT-based & \textbf{41.3} & \textbf{141.2} & \textbf{25.1}          \\ \bottomrule
\end{tabular}
}
\label{tab:coco_sota_metric}
\end{table}

==> tables/BVLT_efficiency.tex <==
\begin{table}[t!]
\caption{Training and inference time comparison of BVLT and VINVL for image captioning.}
\centering
\setlength\heavyrulewidth{1.5pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
Model & VINVL & IMT-1 (Ours) \\
\midrule \midrule
Faster R-CNN (sec/img) &
0.842 (x1.00) &
0.741 (x1.14) \\
\midrule
RSA (sec/img) &
0.027 (x1.00) &
0.017 (x1.59) \\
\midrule
LSA (sec/img) &
0.251 (x1.00) & 
0.143 (x1.76) \\
\midrule
Inference Cost (sec/img) &
1.120 (x1.00) & 
0.901 (x1.24) \\
\midrule
Training Cost (GPU-hour) &
457.86 (x1.00) &
369.60 (x1.24) \\
\bottomrule
\end{tabular}
}
\label{tab:efficiency}
% \vspace{0.3cm}
\end{table}

% \begin{table}[t!]
% % \caption{Effect of [IMT] token on training and inference speed. The numbers in parentheses indicate speed-up ratios.} % \caption
% \caption{Training and inference time comparison of BVLT and VINVL.}
% \centering
% \setlength\heavyrulewidth{1.5pt}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
% Model & 
% % \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Faster R-CNN\\ (sec/img)\end{tabular}} &
% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}RSA\\ (sec/img)\end{tabular}} &
% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}LSA\\ (sec/img)\end{tabular}} &
% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Inference Cost\\ (sec/img)\end{tabular}} &
% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Training Cost\\ (GPU-hour)\end{tabular}} \\ 
% \midrule \midrule
% VINVL & 
% % 0.842 (x1.00) & 
% 0.027 (x1.00) & 0.251 (x1.00) & 1.120 (x1.00) & 457.86 (x1.00) \\
% \midrule
% \textbf{IMT-1 (Ours)} & 
% % 0.741 (x1.14) & 
% 0.017 (x1.59) & 0.143 (x1.76) & 0.901 (x1.24) & 369.60 (x1.24) \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:efficiency}
% % \vspace{0.3cm}
% \end{table}

% \begin{table}[t!]
% % \caption{Effect of [IMT] token on training and inference speed. The numbers in parentheses indicate speed-up ratios.} % \caption
% \caption{Training and inference speedups of BVLT compared to VINVL.}
% \centering
% \setlength\heavyrulewidth{1.5pt}
% \resizebox{0.7\textwidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
% Model Size & Model & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Faster R-CNN\\ (sec/img)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cross Modal Layers\\ (sec/sequence)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Training Cost\\ (GPU-hour)\end{tabular}} \\ \midrule \midrule
% \multirow{2}{*}{BASE}  & VINVL & 0.842 (x1.00) & 0.269 (x1.00) &                                                                                    \\  \cmidrule{2-5}
%                       & \textbf{BVLT (Ours)} & 0.741 (x1.14) & 0.161 (x1.67) &                                                                           \\ \midrule
% \multirow{2}{*}{LARGE} & VINVL & 0.842 (x1.00) & 0.761 (x1.00) &                                                                                    \\ \cmidrule{2-5} 
%                       & \textbf{BVLT (Ours)} & 0.741 (x1.14) & 0.555 (x1.37)&
%                       \\ \bottomrule
% \end{tabular}
% }
% \label{tab:efficiency}
% \end{table}

==> tables/BVLT_nocaps.tex <==
\begin{table}[t]
% \caption{Evaluation on NOCAPS validation sets.} % \caption
\caption{Image captioning performance on NOCAPS validation set.}
\centering
\setlength\heavyrulewidth{1.5pt}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{entire} & \multicolumn{2}{c}{in-domain} & \multicolumn{2}{c}{near-domain} & \multicolumn{2}{c}{out-domain} \\ \cmidrule(l){2-9} 
                       & CIDEr       & SPICE      & CIDEr        & SPICE        & CIDEr     & SPICE    & CIDEr    & SPICE    \\ \midrule \midrule
OSCAR             & 83.4        & 12.0       & 81.6         & 12.0         & 77.6      & 10.6     & 81.1     & 11.7     \\ \midrule
VINVL             & 89.1        & 12.9       & 96.8         & 13.7         & 89.5      & 13.1     & 86.7     & 11.6     \\ \midrule
\textbf{BVLT (Ours)} & 88.0        & 12.6       & 93.1         & 13.2         & 87.7      & 12.8     & 85.0     & 11.6     \\ \bottomrule
\end{tabular}
}
\label{tab:nocaps_metrics}
\end{table}

==> tables/analysis_compare.tex <==
\begin{table}[t!]
    \caption{Performance comparison of different VL downstream training methods.}
    \vspace{-0.1cm}
    \centering
    \setlength\heavyrulewidth{1.5pt}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{} & \multicolumn{3}{c}{COCO test} & \multicolumn{2}{c}{VQAv2 valid}           \\
        \cmidrule(l){2-4} \cmidrule(l){5-6}
        & B4 & C & S & Acc1 & \multicolumn{1}{c}{Acc5} \\
        \midrule
        \midrule
        Zero-shot & 4.0 & 21.0 & 8.0 & - & - \\
        % \midrule
        Linear-probing & - & - & - & 72.7 & 92.8 \\
        % \midrule
        Fine-tuning & 40.4 & 137.2 & 24.5 & 74.1 & 90.1 \\
        % \midrule
        Prefix-tuning & 37.3 & 122.5 & 22.2 & 73.8 & 93.1 \\
        \midrule
        \textbf{CGTL} & \textbf{41.3} & \textbf{141.2} & \textbf{25.1} & \textbf{75.2} & \textbf{93.3} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:comp}
    \vspace{-0.4cm}
\end{table}

==> tables/analysis_imt.tex <==
\begin{table}[h]
    \caption{The effect of P2F-tuning on the image captioning performance. N denotes the random noise vector insertion instead of learned prefix.}
    \centering
    \setlength\heavyrulewidth{1.5pt}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \multirow{2}{*}{Model} & \multicolumn{2}{c}{With prefix} & \multicolumn{3}{c}{COCO Test} \\
        \cmidrule{2-6}
        & Train & Inference & B4 & C & S \\
        \midrule \midrule
        M0 & X & X & 40.7 & 138.8 & 24.6 \\
        M1 & O & X & 22.9 & 75.0 & 15.3 \\
        M2 & O & N & 25.1 & 82.9 & 16.2 \\ 
        % M3 & O & O & 40.8 & 140.3 & 24.9 \\ 
        \midrule \midrule
        M4 (P2F-1) & O & O & 41.1 & 141.0 & 25.0 \\
        \bottomrule
    \end{tabular}}
    \label{tab:ablation_prefix0}
\end{table}

==> tables/analysis_num.tex <==
% \begin{table}[h]
%     \caption{The effect of the number of prefix on IC.}
%     \centering
%     \setlength\heavyrulewidth{1.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \#Prefix &  1 & 2 & 4 & 8 & 16 \\
%         \midrule \midrule
%         BLEU-4  & 40.9 & 41.0 & 41.0 & 41.0 & 41.3 \\ \midrule
%         CIDEr  & 140.7 & 140.2 & 140.3 & 140.4 & 141.2\\ \midrule
%         SPICE  & 25.0 & 25.0 & 25.0 & 24.9 & 25.1 \\
%         \bottomrule
%     \end{tabular}}
%     \label{tab:analysis_num}
% \end{table}

\begin{table}[h]
    \caption{The effect of the number of prefixes on IC.}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \#Prefix &  1 & 2 & 4 & 8 & 16 \\
        \midrule \midrule
        BLEU-4  & 40.9 & 41.0 & 41.0 & 41.0 & 41.3 \\ \midrule
        CIDEr  & 140.7 & 140.2 & 140.3 & 140.4 & 141.2\\ \midrule
        SPICE  & 25.0 & 25.0 & 25.0 & 24.9 & 25.1 \\
        \bottomrule
        & & & & & \\
        & & & & & \\
        & & & & & \\
    \end{tabular}
    }
    \label{tab:prefix_len}
\end{table}

% \begin{table*}[t!]
%     % \caption{The ablation of P2F-tuning.}
%     \setlength\heavyrulewidth{1.5pt}
%     \renewcommand{\arraystretch}{1.2}
%     \begin{minipage}{0.5\textwidth}
%     \caption{Comparison with different tuning methods.}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \multirow{2}{*}{} & \multicolumn{3}{c}{COCO test} & \multicolumn{2}{c}{VQA v2 validation}           \\
%         \cmidrule(l){2-4} \cmidrule(l){5-6}
%         & B4 & C & S & Acc1 & \multicolumn{1}{c}{Acc5} \\
%         \midrule
%         \midrule
%         Zero-shot & 4.0 & 21.0 & 8.0 & - & - \\
%         \midrule
%         Linear-probe & - & - & - & 72.7 & 92.8 \\
%         \midrule
%         Fine-tuning & 40.1 & 139.3 & 24.9 & 74.1 & 90.1 \\
%         \midrule
%         Prefix-tuning & 37.3 & 122.5 & 22.2 & 73.8 & 93.1 \\
%         \midrule
%         \textbf{P2F-tuning (ours)} & \textbf{41.3} & \textbf{141.2} & \textbf{25.1} & \textbf{75.0} & \textbf{93.3} \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:comp}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.45\textwidth}
%     \caption{The effect of the number of prefixes on IC.}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         \#Prefix &  1 & 2 & 4 & 8 & 16 \\
%         \midrule \midrule
%         BLEU-4  & 40.9 & 41.0 & 41.0 & 41.0 & 41.3 \\ \midrule
%         CIDEr  & 140.7 & 140.2 & 140.3 & 140.4 & 141.2\\ \midrule
%         SPICE  & 25.0 & 25.0 & 25.0 & 24.9 & 25.1 \\
%         \bottomrule
%         & & & & & \\
%         & & & & & \\
%         & & & & & \\
%     \end{tabular}
%     }
%     \label{tab:prefix_len}
%     \end{minipage}
% \end{table*}

==> tables/attn_map_model_metric.tex <==
\begin{table}[]
\setlength\heavyrulewidth{1.5pt}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cc|cccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Method} & \multicolumn{8}{c}{Metric}                                           \\
                       & \begin{tabular}[c]{@{}c@{}}OSCAR \\ Pretraining\end{tabular} & \begin{tabular}[c]{@{}c@{}}COCO Caption\\ Finetunning\end{tabular} & Bleu 1 & Bleu 2 & Bleu 3 & Bleu 4 & Meteor & Rouge L & CIDEr & SPICE \\ \hline\hline
M0 & O & O & 0.78 & 0.62 & 0.49 & 0.38 & 0.30 & 0.59 & 1.27 & 0.23 \\
M1 & X & O & 0.74 & 0.57 & 0.44 & 0.34 & 0.29 & 0.56 & 1.15 & 0.22 \\
M2 & O & X & 0.29 & 0.15 & 0.08 & 0.04 & 0.11 & 0.22 & 0.21 & 0.08\\ \bottomrule
\end{tabular}
}
\caption{Metrics of different model training configurations in image captioning.} % \caption
\label{tab:attn_map_model_metric}
\end{table}

==> tables/flickr.tex <==
\begin{table}[t]
\caption{Performance comparison of various VL models on flickr30k test split. SCST is not conducted for this experiments.}
\centering
\setlength\heavyrulewidth{1.5pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
Model       & B4    & C    & S    \\ \midrule \midrule
GVD ~\cite{zhou2019grounded}        & 27.3  & 62.3 & 16.5 \\ \midrule
Unified VLP ~\cite{zhou2020unified} & 30.1  & 67.4 & 17   \\ \midrule
VINVL ~\cite{zhang2021vinvl}        & 35.43 & 87.3 & 21.1 \\ \midrule \midrule
\textbf{P2F-1 (Ours)}               & 36.41 & 90.1 & 21.1 \\ \bottomrule
\end{tabular}}
\label{tab:flickr_metric}
\end{table}


==> tables/imt_cosine_sim.tex <==
\begin{table}[t]
\caption{Cosine similarity between IMT-16 and caption/image tokens.}
\centering
\setlength\heavyrulewidth{1.5pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{cccc|cccc}
\toprule
\multicolumn{4}{c|}{Image} & \multicolumn{4}{c}{IMTs} \\ \midrule
Max & Min & Average & Std & Max & Min & Average & Std \\ \midrule
0.17 & 1.E-08 & 0.03 & 0.02 & 0.16 & 1.E-08 & 0.08 & 0.04 \\ \bottomrule
\end{tabular}
}
\label{tab:imt_cos_similarity}
\end{table}

==> tables/mask_attention_metrics.tex <==
\begin{table}[t]
\setlength\heavyrulewidth{1.5pt}
\caption{Ablation on the attention masking on the converged image tag-based VL model.
X/Y implies that attention map is masked so that X (in query) \textit{cannot} attend Y (in key).}
\vspace{0.2cm}
\centering
\resizebox{0.78\textwidth}{!}{
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Metric} & \multirow{2}{*}{Original Score} & \multicolumn{6}{c}{Attention Masking} \\ \cmidrule(l){3-8} 
&  & C/T  & C/I & T/T & T/I & I/T & I/I \\ \midrule \midrule
BLEU-4  & 41.16  & 41.20 & 21.62 & 20.19 & 40.84  & 20.82  & 30.84  \\ \midrule
METEOR  & 30.94  & 30.90 & 20.96 & 19.51 & 30.91  & 20.12  & 27.29  \\ \midrule
ROUGE-L & 60.96  & 61.00 & 46.85 & 45.56 & 60.82  & 46.20  & 54.42  \\ \midrule
CIDEr   & 139.20 & 139.30 & 75.46 & 60.92 & 138.77 & 68.77 & 107.73 \\ \midrule
SPICE   & 24.77  & 24.72 & 13.38 & 12.75 & 24.73  & 13.52  & 21.34 \\ \bottomrule
\label{tab:attn_mask_attn_metric}
\end{tabular}
}
\end{table}


% \begin{table}[t]
% \setlength\tabcolsep{3pt} % default value: 6pt
% \begin{subtable}[t]{0.52\textwidth}
% \caption{}
% \setlength\heavyrulewidth{1.5pt}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% \multirow{2}{*}{Metric} & \multirow{2}{*}{Original Score} & \multicolumn{6}{c}{Mask Attention} \\ \cmidrule(l){3-8} 
% &  & C/T  & C/I & T/T & T/I & I/T & I/I \\ \midrule \midrule
% BLEU-4  & 41.16  & 41.20 & 21.62 & 20.19 & 40.84  & 20.82  & 30.84  \\ \midrule
% METEOR  & 30.94  & 30.90 & 20.96 & 19.51 & 30.91  & 20.12  & 27.29  \\ \midrule
% ROUGE-L & 60.96  & 61.00 & 46.85 & 45.56 & 60.82  & 46.20  & 54.42  \\ \midrule
% CIDEr   & 139.20 & 139.30 & 75.46 & 60.92 & 138.77 & 68.77 & 107.73 \\ \midrule
% SPICE   & 24.77  & 24.72 & 13.38 & 12.75 & 24.73  & 13.52  & 21.34 \\ \bottomrule
% \end{tabular}
% }
% \end{subtable}
% \hfill
% \begin{subtable}[t]{0.46\textwidth}
% \caption{}
% \setlength\heavyrulewidth{1.5pt}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccc}
% \hline
% \toprule
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mask\\ C/T \& T/I\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Delete\\ All Tags\end{tabular}} & \multicolumn{5}{c}{Metric}                 \\ \cmidrule{3-7} 
%                                                                              &                                                                            & BLEU-4 & METEOR & ROUGE-L & CIDEr  & SPICE \\ \midrule \midrule
% X                                                                            & X                                                                          & 41.16  & 30.94  & 60.96   & 139.20 & 24.77 \\ \midrule
% O                                                                            & X                                                                          & 40.87  & 30.82  & 60.79   & 138.60 & 24.59 \\ \midrule
% X                                                                            & O                                                                          & 41.14  & 30.95  & 61.03   & 139.00 & 24.65 \\ \midrule
% O                                                                            & O                                                                          & 40.66  & 30.77  & 60.62   & 138.03 & 24.41 \\ \midrule
% \end{tabular}
% }
% \end{subtable}
% \caption{(a) Metrics of image captioning tasks when attention is partially masked. (b) Ablations of the masking C/T and T/I attention and deletion of all tags except for [SEP] token in tag sequence. Clearly, attention of C/T and T/I does not affect on performance in this model and I/T is more important then self attention I/I.} % \caption
% \label{tab:attn_mask_attn_metric}
% \end{table}

==> tables/rank_reduction.tex <==
\begin{table}[t]
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{6}{c}{Remaining Rank of Vision Embedding (Ratio)} \\
\cmidrule
                       & 3\%     & 15\%     & 30\%     & 50\%     & 70\%     & 100\%    \\
\cmidrule
\cmidrule
$\text{VINVL}_{\text{BASE}}$            & 31.7    & 118.0    & 134.3    & 138.3    & 139.8    & 140.4    \\
\cmidrule
$\text{OFA}_{\text{BASE}}$              & 13.8    & 22.8     & 130.5    & 144.0    & 146.0    & 146.3 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/vl_models_comparison.tex <==
\begin{table*}[t!]
\centering
\caption{Comparisons of model architectures and pre-training objectives between VL models.}
\setlength\heavyrulewidth{1.5pt}
\aboverulesep=0ex % Solution part 1 of 3
\belowrulesep=0ex % Solution part 1 of 3
    \resizebox{0.85\textwidth}{!}{
        \begin{tabular}{c|c|c|c|c|c|c}
        \toprule 
        \rule{0pt}{1.1EM}
        \multirow{2}{*}{Model} & 
        \multicolumn{3}{|c|}{Model Architecture} & 
        \multicolumn{3}{c}{Pre-training Objectives} \\ \cmidrule{2-7}
        & \begin{tabular}[c]{@{}c@{}}Image\\ Encoder \end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}Text \\ Encoder \end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}VL Fusion\\ Network\end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}Masked \\ Language \\ Modeling\end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}Image \\ Captioning\end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}Contrastive \\ Learning\end{tabular} \\ 
        \midrule \midrule 
        \rule{0pt}{1.1EM}
        LXMERT & Resnet & \multicolumn{2}{|c|}{Shared Transformer Encoder} & O & X & O \\ \midrule 
        \rule{0pt}{1.1EM}
        OSCAR  & Resnet & \multicolumn{2}{|c|}{Shared Transformer Encoder} & O & X & O \\ \midrule 
        \rule{0pt}{1.1EM}
        VINVL  & ConvNext & \multicolumn{2}{|c|}{Shared Transformer Encoder} & O & X & O \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        LEMON  & ConvNext & \multicolumn{2}{|c|}{Shared Transformer Encoder} & O & X & O \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        X-VLM  & ViT & Transformer Encoder & Transformer Decoder & O & X & O \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        SIMVLM & \multicolumn{2}{|c|}{Shared Transformer Encoder} & Transformer Decoder & X & O & X \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        VLMO   & \multicolumn{3}{|c|}{Shared Transformer Encoder} & O & X & O \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        OFA    & Resnet & Transformer Encoder & Transformer Decoder & X & O & O \\ \midrule 
        \rule{0pt}{1.1EM}
        CoCa   & ViT & Transformer Encoder & Transformer Decoder & X & O & O \\ 
        \midrule 
        \rule{0pt}{1.1EM}
        BEiT3  & \multicolumn{3}{|c|}{Shared Transformer Encoder} & O & X & O \\
        \bottomrule 
\end{tabular}}
\label{tab:vl_models_comp}
\end{table*}

==> tables/vqa.tex <==
\begin{table}[h]
\caption{The effect of [IMT] on visual question answering (VQA).}
\centering
\setlength\heavyrulewidth{1.5pt}
\resizebox{0.55\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{VINVL} & \multicolumn{2}{c}{BVLT-1}                 \\ \cmidrule{2-3} 
                       & Inference with IMT & Inference without IMT \\ \midrule \midrule
75.16 \%                  & 74.65 \%             & 74.58 \%                 \\ \bottomrule
\end{tabular}
}
\label{tab:vqa}
\end{table}
